Numerical Pruning for Efficient Autoregressive Models

Transformers have emerged as the leading architecture in deep learning, proving to be versatile and highly effective across diverse domains beyond language and image processing. However, their impressive performance often incurs high computational costs due to their substantial model size. This paper focuses on compressing decoder-only transformer-based autoregressive models through structural weight pruning to improve the model efficiency while preserving performance for both language and image generation tasks. Specifically, we propose a training-free pruning method that calculates a numerical score with Newton's method for the Attention and MLP modules, respectively. Besides, we further propose another compensation algorithm to recover the pruned model for better performance. To verify the effectiveness of our method, we provide both theoretical support and extensive experiments. Our experiments show that our method achieves state-of-the-art performance with reduced memory usage and faster generation speeds on GPUs.

==> sections/10-rebuttal.tex <==




\section*{Reviewer AHAB (5)}


\subsection*{Rebuttal 1}
\subsubsection{Weakness}
This approach is transformer specific, and can not easily adopt to other architectures. Meanwhile, its implementation would require significant efforts from the users.

\subsubsection{Rebuttal}
% \jx{Thank you for reviewing our paper and providing valuable suggestions.}

% We highlight that our method is not Transformer specific. (i) Our method is designed based on  linear layers, as demonstrated in our theoretic analysis  in Lemma 1 and problem formulation in Equation (3) and (9), which investigates the pruning of linear layers.  It is also easy to extend our method for convolutional layers, as the convolution operation can be implemented with linear layers through flatten and unfold operations [1]. Since linear and convolution layers are widely adopted in various models, our method can be applied for a broad range of models such as Transformers and CNNs. (ii) In our paper, we mainly apply our method for Transformers as most layers in Transformers are the computation intensive linear layers, which is a perfect match with our method. Furthermore, it is challenging to prune the Transformers  with billions or tens of billions of parameters in language and vision tasks. Besides, we can make a fair comparison with baselines such as LLM-pruner and FLAP on the same Transformers. 

Thanks for review. We highlight our method is not Transformer specific. (i) It is designed based on linear layers, as outlined in Lemma 1 and detailed in Equations (3) and (9). (ii) We apply our method to LLMs because their computation-intensive linear layers align well with our approach.


% Our implementation is not too complex, and it requires less data and computation resources. (i) The numerical score can be obtained following Algorithm 1 and the weight compensation can be obtained following Equation (11). In algorithm 1 and Equation (11), the most computation intensive operation is  matrix inversion with a computational complexity of $O(D^3)$,  which is common across many LLM pruning methods (such as  SparseGPT) as discussed in Section 3.5. The other operations are just matrix multiplications. The complexity of our method is not very high. (ii) Although our  derivation and analysis  may seem to be complex,  our conclusions are relatively simple with detailed instructions in Algorithm 1 and Theorem 3 with remarks to guide how to obtain the numerical score and weight compensation. We will release our code  to facilitate easy adoption. (iii)  Our method requires much less data and computation resources.  We only need 128 samples to finish the pruning while other methods require much more data such as LLM-Pruner with the whole finetuning dataset and SliceGPT with 1024 samples. Our method  requires  only one single GPU, as we  only need to load and prune a single linear layer at a time without the need to process the whole model. Our method is quite efficient to finish the pruning of a 65B model on a single GPU within a few GPU hours. 

% [1] An Equivalence of Fully Connected Layer and Convolutional Layer

Our implementation is not complex. (i) Algorithm 1 generates numerical score and Equation (11) enables weight compensation. (ii) Our method uses only 128 calibration samples and 1 GPU even for 65B model.
% , while other methods require more data such as LLM-Pruner with whole finetuning dataset and SliceGPT with 1024 calibration samples. (iii) Code will be released to facilitate easy adoption.





%Our method is designed specifically for linear layers, extending beyond transformer-based models and enabling broad applicability across various architectures that incorporate linear layers. Demonstrated in both language and vision models, this approach functions as a plug-and-play solution that integrates seamlessly into any model’s linear layers, requiring only minimal calibration data and minimal setup effort for users. We will release the code publicly to facilitate easy adoption. We will rewrite the our content of the paper to focus on the transformer-based autoregressive models in our revision.




\subsection*{Rebuttal 2}
\subsubsection{Weakness}
Pruned results are not satisfactory. After making such additional efforts, the users would expect significant improvement. However, even under low 20\% pruning ratio, the performance degrades a lot. This raised my concern regarding pruning LLM research. In my opinion, pruning techniques should focus on how to get a smaller model with competitive even better performance to the full model.

\subsubsection{Rebuttal}
% We highlight that our post-training pruning method and other related baselines do not finetune the pruned model. 
% Following SparseGPT, we further investigate post-training structural pruning and compare with other SOTA post-training structural pruning methods such as SliceGPT and FLAP. Since we do not finetune the pruned model in post-training pruning, it is reasonable that the accuracy drops quickly when the sparsity increases, which are also observed in baselines such as LLM-pruner and FLAP. But our method can still achieve non-marginal improvements than SOTA baselines for various large models on language modeling  and image generation  tasks as shown in Table 1, 2, and 3. 

Thanks for review. We note that post-training pruning methods and related baselines do not finetune the pruned models, leading to accuracy drops as sparsity increases, which is consistent with observations in other SOTA methods like LLM-pruner and FLAP. 
% While achieving 90\% sparsity with competitive performance is feasible in CNNs, this is not true for LLMs. 
Meanwhile, SparseGPT shows large accuracy loss at 60\% sparsity in unstructured pruning. It is more challenging for structural pruning even when finetuning is used to maintain performance with 20\% sparsity (see Table 1 of LoRAShear and LLM-pruner, and Table 6 of ShortGPT). 
% Meanwhile, finetuning requires substantial data and computational resources, especially for LLaMA-65B. 
Our work performs much better than baselines and takes a step forward towards a smaller model with competitive performance to dense model.
% We will keep investigating this.


% Further finetuning can improve the performance of pruned models. But finetuning has a number of limitations such as the huge data and computation resource requirements, especially for large models with billions of parameters, as detailed in our response to the finetuning issue.  Due to the huge resource requirement for finetuning, we do not investigate or experiment with finetuning in this paper, and only compare with other post-training pruning methods without finetuning. 

% While it may be easy to achieve a competitive performance with 99\% sparsity in CNNs, it is not the case for LLMs. For the post-training unstructural pruning, SparseGPT demonstrates that the accuracy suffers from  significant loss at 60\% sparsity. For structural pruning, it is also very hard even for the finetuning based methods to remain competitive performance to the dense model under 20\% sparsity (see Table 1 of LoRAShear and LLM-pruner, and Table 6 of ShortGPT). 

% We agree with the reviewer. Our work already performs significantly better than baselines and takes a step forward towards  a smaller model with competitive performance to the dense model. We will keep investigating this. 
%We agree with the reviewer and our work targets to obtain a smaller model achieving competitive performance to the dense  model. We already performs significantly better than baselines and we will keep investigating this.  

%The proposed method is structural pruning method, which can prune a model and get a smaller model. The results generated by our method with 20\% pruning ratio on WikiText2, PTB, and C4 dataset are better than all the other state-of-the-art methods as shown in Table 1 and Table 2.
%\textcolor{red}{todo: take other works as example, say the degration of model performance, say recover with lora finetune is not our focus in this paper.}
%\textcolor{red}{@pu, maybe write more about this rebuttal}

















\subsection*{Rebuttal 3}
\subsubsection{Weakness}
Upon the performance is not there, having fine-tuning stage is necessary to retain the performance.

\subsubsection{Rebuttal}
We agree that finetuning recovers pruned model performance. While finetuning has limitations: (i) massive data and computation resources. ShearedLLaM use 16 GPUs for finetuning on RedPajama with 1.2 trillion tokens. Due to limited resource, it only experiments with small LLMs (1B or 3B). (ii) LoRA may be adopted to reduce cost, it still requires a lot high-quality data and thus long time. LoRAPrune uses LaMini dataset with 2.58M pairs of instructions. (iii) LoRA may perform worse compared with full parameter finetuning as demonstrated in Table 6 of the Wanda paper.


% We agree that the fine-tuning can recover the pruned model performance. However, fine-tuning typically has a number of limitations especially for LLMs with billions of parameters.  (i) Finetuning requires massive data and computation resources (GPUs) especially for LLMs. For example, ShearedLLaM use 16 GPUs  for contined pre-training/finetuning on RedPajama with 1.2 trillion training tokens. Due to the limited resource, it can only experiment with small LLMs of 1B or 3B parameters. 
% (ii) Although certain parameter efficient finetuning methods  such as LoRA may be adopted to reduce the finetuning cost,  it still requires massive high-quality data and thus long finetuning time. For example, Although LLM-pruner and LoRAPrune  can finetune a 65B model with less GPUs, they still require to use massive high quality data, such as the  LaMini instruction dataset used in LoRAPrune with 2.58M pairs of instructions. Table 12 of LLM-pruner demonstrates that more finetuning samples lead to a better accuracy performance, with increased finetuning cost. 
% (iii) Furthermore, LoRA finetuning may perform worse compared with full parameter finetuning as demonstrated in Table 6 of the Wanda paper, due to the limited  number of finetuned parameters. 

% Different from the above finetuning based pruning methods, we investigate post-training pruning following SparseGPT, which only requires a small set of calibration samples to finish the pruning without finetuning.  We can prune a 65B model with a few calibration data  (128 samples) on a single GPU with a few GPU hours, achieving non-marginal perplexity and accuracy improvements compared with SOTA post-training pruning baselines (see Table 1). Our data and computation resource requirements are significantly lower than finetuning based pruning methods. Our method is compatible with finetuning and we can continue to finetune our pruned model for further accuracy  improvements. 




% To further demonstrate our advantages, in the following table, we compare with  the LoRAPrune [4] which adopts fine-tuning on LaMini instruction dataset [1] with 2.58M pairs of instructions. The perplexity results are evaluated with LLaMA-7B on WikiText2 dataset in 2048 sequence length. As demonstrated, our method can achieve better performance than LoRAPrune without fine-tuning on additional data. The reason may be the inappropriate finetuning dataset and the limited number of finetuned parameters with LoRA. 

We provide LLaMA-7B experiments on WikiText2 compared to LoRAPrune [4] which finetuned on LaMini dataset with 2.58M pairs of instructions. 
% Our method achieves better performance.

\begin{table}[h]
\begin{tabular}{cccc}
\toprule
Prune Ratio & 20\% & 30\% & 50\%  \\
\midrule
LoRAPrune   & 7.63 & 8.79 & 11.60 \\
Ours        & \textbf{6.60} & \textbf{7.56} & 11.66 \\
\bottomrule
\end{tabular}
\end{table}

Meanwhile, our method is compatible with finetuning and we provide more results with LLaMA-7B fine-tuning in 2048 length in table as below.
% | Method           | Sparsity | Wiki ↓ | PTB ↓ |
% |------------------|------------------|-----------|-----|
% | LLM-Pruner       | 20%              | 10.73     | 59.73    |
% | LLM-Pruner (LoRA)| 20%              | 8.41      | 41.78    | 
% | Ours             | 20%              | 6.60  | 35.75| 
% | Ours (LoRA)      | 20%              | 6.52      | 34.32    | 
% | LLM-Pruner       | 50%              | 126.02    | 460.71   | 
% | LLM-Pruner (LoRA)| 50%              | 51.56     | 198.76   | 
% | Ours             | 50%              | 11.66 | 82.55| 
% | Ours (LoRA)      | 50%              | 11.34     | 78.48    | 












\subsection*{Rebuttal 4}
\subsubsection{Weakness}
References and compared baselines are not (strongly) enough. I recommend to discuss and compare with more, e.g., LoRAPrune, LoRAShear, ShortGPT, ShearedLLaMA, etc.

\subsubsection{Rebuttal}
% We additionally present comparisons with ShortGPT [5]. We exclude ShearedLLaMA [7] due to its reliance on RedPajama [2] which involves over 1.2 trillion training tokens, LoRAShear [6] due to its reliance on Alpaca [3] dataset which consists 52,000 instructions, and LoRAPrune [4] due to its reliance on LaMini instruction dataset [1] with 2.58M pairs of instructions.
% We present 27\% pruning ratio results with LLaMA2-7B on BoolQ, PIQA, Hella Swag, WSC, and MMLU datasets with the same evaluation pipeline in the following table. The results show that our method performs better.

We provide 27\% pruning ratio results with LLaMA2-7B comparison with ShortGPT [5] in table below. We exclude ShearedLLaMA [7] due to its reliance on RedPajama [2] which involves over 1.2 trillion training tokens, LoRAShear [6] due to its reliance on Alpaca [3] dataset which consists 52,000 instructions, and LoRAPrune [4] due to its reliance on LaMini [1] instruction dataset with 2.58M pairs of instructions.

% \textcolor{red}{todo: eval results on those datasets}
\begin{table}[]
\begin{tabular}{c|ccccc|c}
\toprule
Method   & BoolQ & PIQA  & HellaSwag & WSC   & MMLU  & Average \\
\midrule
Dense    & 71.62 & 77.91 & 71.26     & 50.00 & 45.39 & 63.236  \\
ShortGPT & 74.71 & 66.43 & 53.02     & 52.46 & 43.96 & 58.116  \\
\midrule
Ours     & 69.37 & 76.34 & 68.92     & 48.93 & 31.29 & \textbf{58.97}  \\
\bottomrule
\end{tabular}
\end{table}




[1] LaMini-LM: A Diverse Herd of Distilled Models from Large-Scale Instructions

[2] Redpajama: An open source recipe to reproduce llama training dataset

[3] Stanford Alpaca: An instruction-following llama model.

[4] LoRAPrune: Structured Pruning Meets Low-Rank Parameter-Efficient Fine-Tuning

[5] ShortGPT: Layers in Large Language Models are More Redundant Than You Expect

[6] LoRAShear: Efficient Large Language Model Structured Pruning and
Knowledge Recovery

[7] Sheared LLaMA: Accelerating Language Model Pre-training via Structured Pruning







\section*{Reviewer o6Rc (6)}



\subsection*{Rebuttal 1}
\subsubsection{Weakness}
The generalizability and stability of the pruned method. According to the proposed method, only about 128 samples from the training dataset of WikiText2 are utilized for pruning. However, such few data samples might not be representative enough to prune large foundation models like LLaMA-65B. Does using different data samples, e.g., different samples from the same or different datasets, cause a definitely different architecture of the final pruned model? Moreover, can using more data samples to compute numerical scores improve the final results?

\subsubsection{Rebuttal}

Thanks for review.

We have conducted ablation study on the number of calibration samples, detailed in Figure 4 and Section 4.4. Results show that our method is robust to the number of calibration samples, with improvements in perplexity becoming marginal beyond 128 samples. Additionally, results for LLaMA-7B using different calibration datasets are in table below. Performance improves when the calibration dataset matches the evaluation dataset.


% We have provided the ablation study of different number of samples used for calibration in Figure 4 and Section 4.4. The results demonstrate that our proposed method is robust to the number of calibration samples, as the number of calibration samples more than 128  only leads to marginal improvements on perplexity. When increasing the calibration sample number from 128 to 1024,  we believe that the pruned model architecture only changes slightly considering the marginal  accuracy improvements.  Thus, we adopt 128 calibration samples  with relatively small computation and data requirements.  
%model performance remains consistent even with a large increase in calibration data.

% To make a fair comparison, we follow previous works such as FLAP to use Wikitext2 as the calibration dataset.  As shown in C.3 of FLAP,  choosing different calibration datasets, e.g. C4 and WikiText2, results in a fluctuation of about ±1\% in average accuracy for  zero-shot tasks. This phenomenon is also observed in replication experiments with other methods that rely on calibration data, like SparseGPT.

% We also provide the results with LLaMA-7B on other calibration datasets in the following table. The results becomes better when the calibration  dataset got from training dataset is same as the evaluation dataset.

% \textcolor{red}{todo: eval with different calibration dataset}
\begin{table}[]
\begin{tabular}{c|ccc}
\toprule
Dataset & Wiki & PTB   & C4   \\
\midrule
Wiki    & 6.60 & 35.75 & 9.49 \\
PTB     & 6.67 & 33.56 & 9.53 \\
c4      & 6.65 & 34.23 & 9.48 \\
\bottomrule
\end{tabular}
\end{table}









\subsection*{Rebuttal 2}
\subsubsection{Weakness}
Why Newton's method but not the simple SGD? According to my knowledge, although Newton's method is more effective in theory, it is more complicated and costly and doesn't perform better in some situations. An experiment should be conducted to verify the necessity of Newton's method.

\subsubsection{Rebuttal}

% \textcolor{red}{@yufa, please say the comparison to sgd, especially discuss the complexity as the analysis in section 3.5. we should say such complexity or computation cost for newton method is general for llm pruning method. we would like to get better results, thus we adopt newton}


% Thank you for your valuable feedback regarding the use of Newton's method over SGD. We address your concerns as follows:
Thank you for your valuable feedback, we address your concerns as follows,

1. The Hessian matrix $H$ in Eq.~(7) depends on both the data $X$ and the weights $W$. Without additional assumptions, neither SGD nor Newton's method can guarantee finding a global optimum, as $H$ may not be positive semi-definite, leading to non-convexity.

2. While SGD has a lower per-iteration cost and converges linearly (approximately 1,000 iterations), Newton's method achieves quadratic convergence, typically requiring around 50 iterations [1]. This makes Newton's method significantly faster in reaching convergence despite its higher per-iteration complexity.

3. The Hessian $H$ is already computed when calculating the gradient $g$ in Eq.~(6). Due to overlapping computations, there is no additional memory or computational overhead in obtaining $H$.

4. Although inverting $H$ has a computational complexity of $O(D^3)$, this cost is common across many LLM pruning methods as discussed in Section 3.5, including the SOTA method SparseGPT. Our approach aims to reduce the overall time required for pruning by leveraging Newton's method to compute the pruning mask more efficiently.


5. We further implement the experiment with SGD method with 20\% pruning ratio for LLaMA-7B model on Wikitext2 dataset, and the results are in the following table. The results show that our method with Newton's method achieve better performance. 



[1] Optimization for machine learning



% \textcolor{red}{todo: exp for sgd}
\begin{table}[]
\begin{tabular}{c|ccc}
\toprule
Method & Wiki & PTB   & C4    \\
\midrule
SGD    & 7.21 & 36.98 & 10.26 \\
Newton & 6.60 & 35.75 & 9.49  \\
\bottomrule
\end{tabular}
\end{table}




\subsection{Rebuttal 3}
\subsubsection{Weakness}
In Table 3, there is a lack of the comparison of SliceGPT.

\subsubsection{Rebuttal}

We provide results of SliceGPT with LlamaGen-XXL (cfg=1.75) in following table. SliceGPT does not perform well on image generation task.  
% The reason may be the limited number of  calibration samples, which is set to the same value as FLAP and our method for a fair comparison. 
%As the SliceGPT requires much more calibration data, the SliceGPT can not achieve good results on image generation task when the number of calibration samples are the same as FLAP and ours method.


% \textcolor{red}{todo: run exp for slicegpt}
\begin{table}[]
\begin{tabular}{cc|cc}
\toprule
Method   & Pruning Ratio & FID $\downarrow$  & IS $\uparrow$    \\
\midrule
SliceGPT & 10\%          & 13.56 & 98.75  \\
FLAP     & 10\%          & 7.87  & 145.25 \\
\midrule
Ours     & 10\%          & 6.09  & 168.96 \\
\midrule
SliceGPT & 20\%          & 72.39 & 4.89   \\
FLAP     & 20\%          & 53.86 & 32.41  \\
\midrule
Ours     & 20\%          & 22.45 & 78.64  \\
\bottomrule
\end{tabular}
\end{table}





==> sections/6-checklist.tex <==

% https://aaai.org/conference/aaai/aaai-25/aaai-25-reproducibility-checklist/

\clearpage

\section*{Reproducibility Checklist}



\subsection*{This paper}


\begin{itemize}
    
    \item Includes a conceptual outline and/or pseudocode description of AI methods introduced (\textcolor{blue}{yes}/partial/no/NA)

    \item Clearly delineates statements that are opinions, hypothesis, and speculation from objective facts and results (\textcolor{blue}{yes}/no)

    \item Provides well marked pedagogical references for less-familiare readers to gain background necessary to replicate the paper (\textcolor{blue}{yes}/no)
    
\end{itemize}



\subsection*{Does this paper make theoretical contributions? (\textcolor{blue}{yes}/no)}

If yes, please complete the list below.

\begin{itemize}

    \item All assumptions and restrictions are stated clearly and formally. (\textcolor{blue}{yes}/partial/no)

    \item All novel claims are stated formally (e.g., in theorem statements). (\textcolor{blue}{yes}/partial/no)
    
    \item Proofs of all novel claims are included. (\textcolor{blue}{yes}/partial/no)
    
    \item Proof sketches or intuitions are given for complex and/or novel results. (\textcolor{blue}{yes}/partial/no)
    
    \item Appropriate citations to theoretical tools used are given. (\textcolor{blue}{yes}/partial/no)
    
    \item All theoretical claims are demonstrated empirically to hold. (\textcolor{blue}{yes}/partial/no/NA)
    
    \item All experimental code used to eliminate or disprove claims is included. (\textcolor{blue}{yes}/no/NA)

\end{itemize}




\subsection*{Does this paper rely on one or more datasets? (\textcolor{blue}{yes}/no)}

If yes, please complete the list below.

\begin{itemize}

    \item A motivation is given for why the experiments are conducted on the selected datasets (\textcolor{blue}{yes}/partial/no/NA)
    
    \item All novel datasets introduced in this paper are included in a data appendix. (yes/\textcolor{blue}{partial}/no/NA)
    
    \item All novel datasets introduced in this paper will be made publicly available upon publication of the paper with a license that allows free usage for research purposes. (\textcolor{blue}{yes}/partial/no/NA)
    
    \item All datasets drawn from the existing literature (potentially including authors’ own previously published work) are accompanied by appropriate citations. (\textcolor{blue}{yes}/no/NA)
    
    \item All datasets drawn from the existing literature (potentially including authors’ own previously published work) are publicly available. (\textcolor{blue}{yes}/partial/no/NA)
    
    \item All datasets that are not publicly available are described in detail, with explanation why publicly available alternatives are not scientifically satisficing. (yes/partial/no/\textcolor{blue}{NA})

\end{itemize}


\subsection*{Does this paper include computational experiments? (\textcolor{blue}{yes}/no)}

If yes, please complete the list below.

\begin{itemize}

    \item Any code required for pre-processing data is included in the appendix. (yes/partial/\textcolor{blue}{no}).
    
    \item All source code required for conducting and analyzing the experiments is included in a code appendix. (yes/\textcolor{blue}{partial}/no)
    
    \item All source code required for conducting and analyzing the experiments will be made publicly available upon publication of the paper with a license that allows free usage for research purposes. (yes/\textcolor{blue}{partial}/no)
    
    \item All source code implementing new methods have comments detailing the implementation, with references to the paper where each step comes from (\textcolor{blue}{yes}/partial/no)
    
    \item If an algorithm depends on randomness, then the method used for setting seeds is described in a way sufficient to allow replication of results. (\textcolor{blue}{yes}/partial/no/NA)
    
    \item This paper specifies the computing infrastructure used for running experiments (hardware and software), including GPU/CPU models; amount of memory; operating system; names and versions of relevant software libraries and frameworks. (\textcolor{blue}{yes}/partial/no)
    
    \item This paper formally describes evaluation metrics used and explains the motivation for choosing these metrics. (\textcolor{blue}{yes}/partial/no)
    
    \item This paper states the number of algorithm runs used to compute each reported result. (\textcolor{blue}{yes}/no)
    
    \item Analysis of experiments goes beyond single-dimensional summaries of performance (e.g., average; median) to include measures of variation, confidence, or other distributional information. (yes/\textcolor{blue}{no})
    
    \item The significance of any improvement or decrease in performance is judged using appropriate statistical tests (e.g., Wilcoxon signed-rank). (yes/\textcolor{blue}{partial}/no)
    
    \item This paper lists all final (hyper-)parameters used for each model/algorithm in the paper’s experiments. (\textcolor{blue}{yes}/partial/no/NA)
    
    \item This paper states the number and range of values tried per (hyper-) parameter during development of the paper, along with the criterion used for selecting the final parameter setting. (\textcolor{blue}{yes}/partial/no/NA)

\end{itemize}












==> sections/trash.tex <==
\Yufa{Make $X$ the input of attention not output.
$X_p \in \R^{N \times D_p}$ is $X \in \R^{N \times D}$ after pruned
$Attn(X) = D^{-1}AV_p$ where $A = \exp(Q_pK_p^\top)$, $D = A \cdot {\bf 1}$ where $Q_p = X W^Q_p$


$Y_p = Attn(X_p) \in \R^{N \times D_p}$ 
$W^o \in \R^{D \times D}$
$W_p^o \in \R^{D_p \times D}$

current $Y W_p^o \approx Y W^o$

we want to $Y_p W_p^o \approx Y W^o$ 
we optimize $W_p^o$
}


% \Yufa{
% \begin{align*}
%     Y = W X, Y_p = (M \circ W) X
% \end{align*}
% We want 
% \begin{align*}
%     & ~ \|Y - Y_p\| \leq \epsilon\\
%     \implies & ~ \|WX - (M \circ W)X\| \leq \epsilon \\
%     \implies & ~ \|W - (M \circ W)\| \cdot \|X\| \leq \epsilon\\
%     \implies & ~ \|W - (M \circ W)\| \cdot \|X\| \\
%     \leq & ~ \|W_{\text{entires we set to 0}}\| \cdot \|X\| \\
%     \implies & ~ R \|W_{\text{entires we set to 0}}\| \leq R \rho ???
% \end{align*}
% for any $X$ and $W_p \in \R^{D \times D}$ but we set some entries to 0. 
% The way we set 0 is by sorted score for one row of score. 
% where $\rho$ is a pruning ratio

% $\|X\| \leq R$ might have some distribution.  

% Extend to all layer.
% 1. all layer will have different prun ratio, some will have small ratio so error not so big
% 2. global sort satisfy our result.

% number of zero entries in mask $=D^2 \rho$
% after nomalization $\|W_{*,j}\|$ we pick the max norm of $D^2 \rho$ entries in $ \|W\|$
% }

\newpage
We construct $X,W$ explicitly.
\subsection{Synthetic Dataset}
For $X \in \R^{N \times D}$, we assume that 
\begin{align*}
    x_{i,j} = 1 + (j-1) \cdot d
\end{align*}
where $d = 1$.
We assume $W \in \R^{D_p \times D}$ is a vector $1 \times D$ as:
\begin{align*}
W = \begin{bmatrix}
    1 & 2 & \dots & D
\end{bmatrix}^\top
\end{align*}

We have
\begin{align*}
    X = \begin{bmatrix}
        1 & 1 & 1 \dots 1 \\
        2 & 2 & 2 \dots 2 \\
          &   & \vdots\\
        N & N & N \dots N 
    \end{bmatrix}
\end{align*}

\begin{align*}
    \mu := \ov{X} = & ~ \frac{1}{N} \sum_{n=1}^N X_{n,*} \in \R^{D}\\
\end{align*}
Since $B=1$, for $\ov{X_n}$, we have
\begin{align*}
    \ov{X_n} = X_n \in \R^{D} 
\end{align*}
We have 
\begin{align*}
     \mu = & ~ 
    \begin{bmatrix}
        (N+1)/2 & (N+1)/2 & \dots & (N+1)/2
    \end{bmatrix}^\top \in \R^{D}
\end{align*}
Then we consider it in $j = 1 \to D$, we have 
\begin{align*}
    y_j = & ~ W_j\\ 
    \sigma _j = & ~ \| y_j \|_2^2
\end{align*}
Then we calculate the score
\begin{align*}
    S = & ~\frac{1}{N} \sum_{n=1}^N (X_n - \mu) \circ W \\
      = & ~ \begin{bmatrix}
        \frac{1(N^2-1)}{2N} & \frac{2(N^2-1)}{2N} & \dots & \frac{D(N^2-1)}{2N}B
      \end{bmatrix} 
\end{align*}





\begin{lemma}\label{lem:f2norm_solution}
     For the problem,
     \begin{align*}
         \min_{X \in \mathbb{R}^{n\times p}} \| A X-B \|_F^2
     \end{align*}
     the optimal $X$ is given by $A^\dagger B$.
     \Yufa{Need to add mask version.}
\end{lemma}

\begin{proof}
    Fix a choice of $A\in \mathbb{R}^{m\times n}, X\in \mathbb{R}^{n\times p}, B\in \mathbb{R}^{m\times p}$ Consider the function $f(X):= \|AX-B\|_F^2$. Minimizing $f$ then solves our problem since $f$ is a convex function, we have that minimum of $f$ happens on a point where
     \begin{align*}
         f'(X)=  \frac{\partial f(X)}{\partial X}=0
     \end{align*}
     Then, by Definition~\ref{def:F_norm}, we have
     \begin{align*}
        f(X) =&~ \|AX-B\|_F^2\\
             =&~\tr[(AX-B)^\top (AX-B)]\\
             % =&~ \tr[(AX)^\top (AX)- (AX)^\top B- B^\top(AX) +B^\top B]\\
             =&~ \tr[X^\top A^\top AX]-\tr[2B^\top AX]+\tr[B^\top B]
     \end{align*}
     Using the rules of gradients, we have
     \begin{align*}
         f'(X)= \frac{\partial f(X)}{\partial X}=2 A^\top AX-2A^\top B
     \end{align*}
     Thus, when $f'(X)=0$, we have
     \begin{align*}
         A^\top AX=&~A^\top B\\
         X=&~(A^\top A)^{-1} A^\top B\\
         X = & ~ A^\dagger B
     \end{align*}
     where the last step follows from the definition of pseudo-inverse (Definition~\ref{def:pseudo_inverse}).
     This gives a closed-form solution.
\end{proof}

% \Yufa{Bo, define Leverage Score.}






\iffalse
\begin{algorithm*}[!ht]\caption{Admm optimization\Bo{original admm optimization}}
\begin{algorithmic}[1]
\Procedure{PruneAlgorithm}{$X \in \mathbb{R}^{n \times d}, W \in \mathbb{R}^{d \times m}, W \in \{0,1\}^{d \times m}, \rho \in \mathbb{R}$}
    \For{$i=1 \to k$}
        \If{$i \leq k_s$}
            \State $s_i \gets s_f \cdot (i/k_s)^3$ 
            \State $M \gets$ Mask lowest $s_i$ indices from $|W+U|$
        \EndIf
    \State $Z \gets (W +U) \circ M$ \Comment{Here $\circ$ is the hadamard product}
    \State $U \gets U + (W - Z)$
    \State $W \gets (X^\top X + \rho I)^{-1}  ( X^\top X W + \rho (Z- U) )$
   \EndFor
   \State \Return $W \gets (W + U) \circ M $
\EndProcedure
\end{algorithmic}
\end{algorithm*}
\fi


\newpage
\textbf{Summary}  Here are some details in Algorithm~\ref{alg:optimze} to accelerate training. 
\begin{itemize}
    \item Line~\ref{line:compute_E} Compute $E \in \mathbb{R}^{D \times D}\gets \sum_{i=1}^B (X_i ^\top X_i)$, where $X_i$ is the $i$-th batch of $X$. $E \in \mathbb{R}^{D\times D}$ is used to capture the eigenrelationships in the $X$.
    \item Line~\ref{line:extract_diagonal} Compute $u \gets {\bf 1}_D / ( \sqrt{\mathrm{Diag}(E)} + \alpha \cdot {\bf 1}_D )$, where $\mathrm{Diag}(E)$ extracts the diagonal elements of $E \in \mathbb{R}^{D\times D}$, which are used to normalize $E \in \mathbb{R}^{D \times D}$. The operation here is entry-division.
    \item Line~\ref{line:diag_W} Update $W \gets W \cdot \mathrm{diag}(u)$ to scale $W$ according to $u$.
    \item Line~\ref{line:addterm_invertible} Add a small diagonal term $E \gets E+ D^{-1}\eta \cdot \cdot \langle \mathrm{Diag}(E), {\bf 1}_D \rangle \cdot I_D$ to make sure that it is invertible.
    \item Line~\ref{line:select_W} This line is used to determine which elements in $W$ need to be updated.
    \item Line~\ref{line:sum_bias} $U$ is the summation of bias, the Lagrange multiplier used to accumulate the difference between $W$ and $Z$ as a way to push $W$ towards updating in the direction that satisfies the constraint $M$.
    \item Line~\ref{line:regulate_WandZ} $\rho$ is a penalty parameter that regulates the effect of $Z$ and $U$ deviations on $W$ updates.
    \item Line~\ref{line:eliminate_redundancy} ensures that only the mask matrix $M$ elements specified in M are retained.
\end{itemize}


\begin{remark}\label{rem:mistake_iter}
    line~\ref{line:mistake_iter} in Algorithm~\ref{alg:optimze}: the goal of using the new notation $\widetilde{E}$ is to avoid the confusion that the following for loop needs to be reversed each time.
\end{remark}

\begin{definition}[Frobenius-norm]\label{def:F_norm}
Suppose we have a vector $A\in \mathbb{R}^{m\times n}$, we can define the Frobenius norm of $A$ as $\| A\|_F:=(\sum_{i=1}^m \sum_{j=1}^n a_{ij}^2)^{1/2}$.
Additionally, we have $\| A\|_F^2 = \tr[A^\top A]$.
\end{definition}

\begin{definition}[Pseudo-inverse]\label{def:pseudo_inverse}
    For a matrix $ A\in \R^{n\times m}$, we have the pseudo-inverse denoted by $A^\dagger := (AA^\top)^{-1}A^\top$.
\end{definition}

\begin{fact}[Derivatives of Trace]\label{fac:matrix_derivative}
For any $X \in \R^{m \times n}$: we have
    $\frac{\partial \tr[F(X)]}{\partial X}= f(X)$,
where $f(\cdot)$ is the scalar derivative of $F(\cdot)$.
\end{fact}



\newpage

\begin{algorithm}[!ht]\caption{Layer importance scoring. This algorithm computes the score  $S$ for one layer.}\label{alg:importance_score}
\begin{algorithmic}[1]
\Procedure{GetScore}{$X\in \mathbb{R}^{B\times N \times D}, W \in \mathbb{R}^{D_p \times D}, B \in \mathbb{N}_+, L \in \mathbb{N}_{+}, D \in \mathbb{N}_+, D_p \in \mathbb{N}_+, N \in \mathbb{N}_+$}   
\State \Comment{$i$ denotes the $i$-th batch}
\State \Comment{$l$ denotes the $l$-th layer}
\State \Comment{$n$ denotes the $n$-th token}
\State \Comment{$k$ denotes the $k$-th channel}
    \State $\overline{X} \gets \frac{1}{BN} \sum^{B}_{i=1} \sum^{N}_{n=1} X_{i,n,*}$ 
    \For{$n=1 \to N$}
    \State $\overline{X}_n =\frac{1}{B} \sum_{i=1}^B X_{i,n,*}$ \Comment{$\overline{X}_n \in \mathbb{R}^{D}$}
    \EndFor
    \State $\mu \gets \overline{X}$ \Comment{$\mu \in \mathbb{R}^D$}
    \For{$j= 1\to D$}
    \State $y_j \gets W_{*, j}$ \Comment{$W_{*,j} \in \mathbb{R}^{D_p}$}
    \State $\sigma_j \gets \| y_j \|_2^2$ \Comment{$\sigma \in \mathbb{R}^D$}
    \EndFor
    \State  $ S \gets \frac{1}{N}  \sum^{N}_{n=1} ( \overline{X}_{n} - \overline{X} ) \circ \sigma$ \Comment{$S\in \mathbb{R}^D$}    
    \State $ S \gets \frac{S - \mu(S)}{\sigma(S)}$
   \State \Return $S$    \Comment{Score for the layer}
\EndProcedure
\end{algorithmic}
\end{algorithm}
\Bo{In wanda, we calculate the score in every specific element in $W$ matrix. We calculate every channel(column) in $W$ matrix. Our method is similar to wanda. We need to read wanda.}\\
\Bo{We can only focus on Algorithm1, the difference between our method and wanda. One element and column?}\\
\Bo{Both of two methods are fast. New proof just modified element $\to$ column.}

\begin{algorithm}[!ht]\caption{Generate mask. This algorithm uses scores of each attention/MLP layer to generate the pruning mask.}\label{alg:sort_globally}
\begin{algorithmic}[1]
\Procedure{GenerateMask}{$L, D, h, \rho, d_{h}\in \mathbb{R} , S \in \mathbb{R}^{L \times D}$} 
    \State \Comment{$L$ denotes the total number of layers}
    \State \Comment{$N$ denotes the total number of tokens}
    \State \Comment{$D$ denotes the number of hidden states}
    \State \Comment{$H$ denotes the number of heads in attention, and $h$ denotes the head index}
    \State \Comment{$S_l \in \R^D$ denotes the scores in $l$-th layer of Attention/MLP}
    % \State \Comment{ $S^{\mathsf{Attn}}$ denotes the score of attention}
    % \State \Comment{$S^{\mathsf{MLP}}$ denotes the score of MLP}
    \State \Comment{$d_{h} := D/H$ denotes the dimension of one head}
    \State \Comment{$\rho$ denotes the pruning ratio}
    \For{$l = 1\to L$}
        \For{$h = 1\to H$}
            \State $S_{l}(h) \gets \sum_{i=(h-1)d_h+1}^{h d_h+1} S_{l,i}/d_h$ 
            \State $S_{l,h} \gets S_l(h)$
        \EndFor
        \State $S_{l} \gets S_{l} \cdot \alpha$ 
        
        \Comment{$\alpha \in \mathbb{R}= 4d_h/3h$ if $S$ is the attention layer, and $\alpha = 1$ if $S$ is the MLP layer} 
    \EndFor
    \State $I \gets \mathrm{Argsort}(S)$ 
    \State $M[I] \gets 0$ \Comment{Set the elements at index $I$ in $M$ to 0}
    \State \Return $M$ \Comment{Pruning mask}
\EndProcedure
\end{algorithmic}
\end{algorithm}


\begin{algorithm}[!ht]\caption{Layer pruning. The algorithm }\label{alg:optimze}
\begin{algorithmic}[1]
\Procedure{PruneAlgorithm}{$X \in \mathbb{R}^{B \times N \times D}, W \in \mathbb{R}^{D_p \times D}, M \in \{0,1\}^{D_p \times D}, k \in \mathbb{N}_+, \rho \in \mathbb{R}, \alpha \in (0,0.1), \eta \in \mathbb{R}, B \in \mathbb{N}_+, N \in \mathbb{N}_+, D \in \mathbb{N}_+$}
    \State \Comment{$X$ denotes input samples}
    \State \Comment{$W$ denotes weight matrix}
     \State \Comment{$M$ denotes pruning mask}
      \State \Comment{We choose $\rho = 10^{-8}$(in practice)  denotes penalty ratio}
     \State \Comment{$\alpha \in (0,0.1)$ denotes normalization constant}
      \State \Comment{$\eta$ is a constant to make $E$ invertible}
    \State {\color{blue}/*Step 1, guarantee matrix is p.s.d*/}
    \State $E \gets \sum_{i=1}^B (X_i ^\top X_i)$ \Comment{$X_i \in \mathbb{R}^{N \times D}$ denotes the $i$-th batch of $X$, $E \in \mathbb{R}^{D \times D}$}\label{line:compute_E}
    %\State \Comment{$E^{\circ}$ denotes $E$ without diagonal entries}
    \State $u \gets {\bf 1}_D / ( \sqrt{\mathrm{Diag}(E)} + \alpha \cdot {\bf 1}_D )$ \Comment{$\mathrm{Diag}(E)$ is a column vector that has length $D$}\label{line:extract_diagonal}
    \State $E \gets \mathrm{diag}(u) E \mathrm{diag} (u)$ \Comment{$\mathrm{diag}(u)$ is turning a vector into a diagonal matrix}\label{line:diagonal_E}
    \State $W \gets W \cdot \mathrm{diag}(u)$ \Comment{$W \in \mathbb{R}^{D_p \times D}$}\label{line:diag_W}
    \State $E \gets E + \eta \cdot \langle \mathrm{Diag}(E) , {\bf 1}_D \rangle \cdot I_D / D$ \Comment{$I_D$ is a $D \times D$ indentity matrix, in practice $\eta=0.1$}\label{line:addterm_invertible}
    \State {{\color{blue}/*The following three matrix variables will be static over the iterations*/}}
    \State $\widetilde{E} \gets E^{-1}$\label{line:mistake_iter}
    \State $F \gets W \cdot E$ \Comment{$F \in \mathbb{R}^{D_p \times D}$}
    \State \Comment{$M$ is static}
    \State {{\color{blue}/*The following three matrix variables will be changed over the iterations*/}}
    \State $U \gets 0^{D_p \times D}$ 
    \State \Comment{$Z \in \mathbb{R}^{D_p \times D}$ will be changed as well}
    \State \Comment{$W \in \mathbb{R}^{D_p \times D}$ will be changed as well}
    \State {\color{blue}/*Step 2. Running ADMM*/}
    % \Yufa{Below are the most important.}
    \For{$i=1 \to k$} \Comment{In practice, we choose $k=20$}
    \State $Z \gets (W +U) \circ M$ \Comment{Here $\circ$ is the hadamard product}\label{line:select_W}
    \State $U \gets U + (W - Z)$\label{line:sum_bias}
    \State $W \gets   (F + \rho (Z- U) ) \widetilde{E}$ \Comment{$\rho = 10$}\label{line:regulate_WandZ}
   \EndFor
   \State \Return $W \gets (W + U) \circ M $ \label{line:eliminate_redundancy}
\EndProcedure
\end{algorithmic}
\end{algorithm}



\iffalse
\begin{lemma}
If the following conditions hold:
\begin{itemize}
    \item Let $W \in \R^{D \times D}$, $X \in \R^{N \times D}$.
    \item Let $M \in [0,1]^{D}$ and $\rho \in [0,1]$ be ratio of number of zeros to number of entries in $M$.
    \item Assume $\|X\| \leq R$. 
\end{itemize}
We want to get the optimal $M$ such that
\begin{align*}
    \underset{M}{\arg \min} & ~~~~ \sum_{i \in [D]} \|X W_i - X(M \circ W_i)\|_2 \\
    \mathrm{subject~to} & ~~~~ {\bf 1}_D^\top M  = (1-\rho)D 
\end{align*}
\end{lemma}

% \Yufa{Not need to get close form, give an algorithm to solve this is good.}
\fi
